On the Role of Diffractive Production in Precision Studies of W and Z Bosons at the LHC

The increasing precision of measurements at the Large Hadron Collider requires a detailed understanding of all contributions to electroweak boson production. We estimate the impact of single-diffractive W and Z production on precision observables at $\sqrt{s}=5$, 7, 8, and 13 TeV. The non-diffractive baseline is calculated with DYTurbo, while Herwig provides the relative single-diffractive contribution and its transverse-momentum dependence. Factorization breaking is incorporated through a $p_T$-dependent rapidity-gap survival probability calculated with the dynamic multiparton-interaction model of Pythia8. The diffractive Asimov spectrum is constructed by deterministic bin-by-bin reweighting of the same high-numerical-precision DYTurbo cross section used for the non-diffractive baseline. With the non-perturbative parameters profiled, the nominal relative shifts in $\alpha_s$ are -0.0072%, -0.043%, -0.070%, and -0.067% at 5, 7, 8, and 13 TeV, respectively. Five Pythia8 Pomeron-flux and diffractive-PDF configurations give a maximum spread of $9.4\times10^{-6}$ in $\Delta\alpha_s$. In the W-mass study, the largest bias from an unmodelled survived single-diffractive contribution is 1.58 MeV, and the largest residual after applying the corresponding model-matched template correction is 1.14 MeV. These shifts are below the relevant fit precision, and no phenomenologically significant impact on $m_W$ is expected within the tested models.

==> svmyepj-spec.tex <==
% SVJour DOCUMENT CLASS OPTION EPJ -- The European Physical Journal Special Topics
%%
%%
%% \CharacterTable
%%  {Upper-case    \A\B\C\D\E\F\G\H\I\J\K\L\M\N\O\P\Q\R\S\T\U\V\W\X\Y\Z
%%   Lower-case    \a\b\c\d\e\f\g\h\i\j\k\l\m\n\o\p\q\r\s\t\u\v\w\x\y\z
%%   Digits        \0\1\2\3\4\5\6\7\8\9
%%   Exclamation   \!     Double quote  \"     Hash (number) \#
%%   Dollar        \$     Percent       \%     Ampersand     \&
%%   Acute accent  \'     Left paren    \(     Right paren   \)
%%   Asterisk      \*     Plus          \+     Comma         \,
%%   Minus         \-     Point         \.     Solidus       \/
%%   Colon         \:     Semicolon     \;     Less than     \<
%%   Equals        \=     Greater than  \>     Question mark \?
%%   Commercial at \@     Left bracket  \[     Backslash     \\
%%   Right bracket \]     Circumflex    \^     Underscore    \_
%%   Grave accent  \`     Left brace    \{     Vertical bar  \|
%%   Right brace   \}     Tilde         \~}
\ProvidesFile{myepj-spec.clo}
              [2006/9/9 v1
      style option for The European Physical Journal Special Topics]
\typeout{SVJour Class option: myepj-spec.clo for The European Physical Journal}
\DeclareOption{leqno}{\input{leqno.clo}}
\let\if@nopacs\iffalse
\DeclareOption{nopacs}{\let\if@nopacs\iftrue}
\ExecuteOptions{final,10pt}
\newif\if@normhead \@normheadtrue
\def\hugehead{\@normheadfalse
\let\ProcessRunnHead=\relax
\onecolumn
\let\thanks=\footnote
\long\def\@makefntext##1{\parindent\bibindent
     \columnwidth\textwidth
     \advance\columnwidth -\columnsep
     \divide\columnwidth\tw@
     \hsize\columnwidth
     \linewidth\columnwidth
     \noindent\hbox to\parindent{\hss\@makefnmark\enspace}##1}%
}
\let\if@mathematic\iffalse
% No size changing allowed, hence a copy of size10.clo is included
\renewcommand\normalsize{%
   \@setfontsize\normalsize\@xpt{10.5dd}%
   \abovedisplayskip 10\p@ \@plus2\p@ \@minus5\p@
   \abovedisplayshortskip \z@ \@plus3\p@
   \belowdisplayshortskip 6\p@ \@plus3\p@ \@minus3\p@
   \belowdisplayskip \abovedisplayskip
   \let\@listi\@listI}
\normalsize
\newcommand\small{%
   \@setfontsize\small\@ixpt{10dd}%
   \abovedisplayskip 8.5\p@ \@plus3\p@ \@minus4\p@
   \abovedisplayshortskip \z@ \@plus2\p@
   \belowdisplayshortskip 4\p@ \@plus2\p@ \@minus2\p@
   \def\@listi{\leftmargin\leftmargini
               \parsep 0\p@ \@plus1\p@ \@minus\p@
               \topsep 8\p@ \@plus2\p@ \@minus4\p@
               \itemsep0\p@}%
   \belowdisplayskip \abovedisplayskip
}
\let\footnotesize\small
\newcommand\scriptsize{\@setfontsize\scriptsize\@viipt\@viiipt}
\newcommand\tiny{\@setfontsize\tiny\@vpt\@vipt}
\newcommand\large{\@setfontsize\large\@xiipt{13dd}}
\newcommand\Large{\@setfontsize\Large\@xivpt{15dd}}
\newcommand\LARGE{\@setfontsize\LARGE\@xviipt{17dd}}
\newcommand\huge{\@setfontsize\huge\@xxpt{25}}
\newcommand\Huge{\@setfontsize\Huge\@xxvpt{30}}
%
\setlength{\textwidth}{145mm}\setlength{\textheight}{220mm}
%
\def\epj@maketitle{\par
\ch@ckobl{journalname}{Noname}
%later}
\ch@ckobl{title}{A title should be given}
\ch@ckobl{author}{Name(s) and initial(s) of author(s) should be given}
\ch@ckobl{institute}{Address(es) of author(s) should be given}
\ch@ckobl{abstract}{Abstract is missing.}
\begingroup
%
    \renewcommand\thefootnote{\@fnsymbol\c@footnote}%
    \def\@makefnmark{$^{\@thefnmark}$}%
    \def\switch@fnmark{\def\thefootnote{\mathrm{\alph{footnote}}}}
%
 \def\lastand{\ifnum\value{inst}=2\relax
                 \unskip{} \andname\
              \else
                 \unskip, \andname\
              \fi}%
 \def\and{\stepcounter{auth}\relax
          \if@smartand
             \ifnum\value{auth}=\value{inst}%
                \lastand
             \else
                \unskip,
             \fi
          \else
             \unskip,
          \fi}%
 \thispagestyle{empty}
 \ifnum \col@number=\@ne
   \@maketitle
 \else
   \@maketitle%
 \fi
 \global\@topnum\z@
 \if@normhead
    \@thanks
 \else
    \vspace{\@tempdima}
    \addtocounter{page}{-1}
    \if!\the\authorrunning!
       \authorrunning{ }%
    \fi
 \fi
 \if!\@mail!\else
    \footnotetext[0]{\kern-\bibindent\mailname\
    \ignorespaces\@mail}%
 \fi
%
 \if@runhead
    \ProcessRunnHead
 \fi
%
 \endgroup
 \setcounter{footnote}{0}
 \global\let\thanks\relax
 \global\let\maketitle\relax
 \global\let\@maketitle\relax
 \global\let\@thanks\@empty
 \global\let\@author\@empty
 \global\let\@title\@empty
 \global\let\@subtitle\@empty
 \global\let\title\relax
 \global\let\author\relax
 \global\let\and\relax}
%
\def\epj@@maketitle{%\newpage
 \normalfont
% \vbox to0pt{\vskip-40pt
% \nointerlineskip
% \makeheadbox\vss}\nointerlineskip
 \if@normhead
    \setbox\authrun=\vbox\bgroup
 \fi
 {\LARGE \sffamily\bfseries
  \hrule\@height\logodepth\@width\z@
  \pretolerance=10000
  \rightskip=0pt plus 4cm
 \if!\@headnote!\else
   \noindent
   {\LARGE\normalfont\itshape\ignorespaces\@headnote\par}\vskip 3.5mm
 \fi
  \noindent\ignorespaces
  \@title \par}\vskip 11.24pt\relax
 \authorfont
 \if!\@subtitle!\else
   {\large\sffamily\bfseries
   \pretolerance=10000
   \rightskip=0pt plus 3cm
   \noindent\ignorespaces\@subtitle \par}\vskip 11.24pt
 \fi
 \lineskip .5em
 \switch@fnmark
 \def\@makefnmark{$^{\mathrm\@thefnmark}$}%
 \protected@xdef\@thanks{\@thanks\protect\switch@fnmark}%
 \setbox0=\vbox{\setcounter{auth}{1}\def\and{\stepcounter{auth} }%
                \hfuzz=2\textwidth\def\thanks##1{}\@author}%
 \setcounter{footnote}{0}%
 \value{inst}=\value{auth}%
 \setcounter{auth}{1}%
 \rightskip=0pt plus 2cm
 \noindent\ignorespaces\@author\vskip7.23pt
 \rightskip=0pt\relax
 \small\rm
 \institutename
 \vskip 12.85pt
 \leftskip=1.5cm\rightskip=\leftskip
 \vskip 12.85pt
 {\topsep=0pt\partopsep=0pt\parsep=0pt\itemsep=0pt\relax
  \def\pacsstart##1##2{##1\hskip5pt plus2ptminus2pt##2}%
  \def\and##1##2{\unskip\ -- ##1\hskip5pt plus2ptminus2pt##2}%
  \trivlist\item[\hskip\labelsep
  {\sffamily\bfseries\abstractname}]%
  \leftskip=1.5cm\rightskip=\leftskip
  \@abstract
  \endtrivlist}%
 \if@normhead
    \egroup % end of header box
    \@tempdima=\headerboxheight
    \advance\@tempdima by-\ht\authrun
    \ifdim\@tempdima>0pt
       \vrule width0pt height\@tempdima
    \fi
    \unvbox\authrun
    \global\@minipagetrue
    \global\everypar{\global\@minipagefalse\global\everypar{}}
 \else
    \typeout{\the\c@auth\space author names and}
    \typeout{\the\c@inst\space institutes processed}
    \global\@tempdima=\pagetotal
    \global\advance\@tempdima by22.47pt
 \fi
 \vskip22.47pt
}
%
\def\epjabstract#1{\gdef\@abstract{#1}}
%
\def\epjrunnhead{\markboth{}{}}%
%
\AtEndOfClass{\let\ackname\@empty
\let\if@runhead\iftrue
\let\if@smartand\iftrue
\let\@maketitle=\epj@@maketitle
\let\maketitle=\epj@maketitle
\let\ProcessRunnHead=\epjrunnhead
\let\abstract=\epjabstract
\def\@evenhead{\small\rlap{\thepage}\hfil\leftmark\hfil}%
\def\@oddhead{\small\hfil\rightmark\hfil\llap{\thepage}}%
\def\sectcounterend{}
\setlength\columnsep{4mm}
\def\section{\@startsection{section}{1}{\z@}%
    {-21dd plus-4pt minus-4pt}{10.5dd plus 4pt
     minus4pt}{\large\sffamily\bfseries\boldmath}}
\def\subsection{\@startsection{subsection}{2}{\z@}%
    {-21dd plus-4pt minus-4pt}{10.5dd plus 4pt
     minus4pt}{\normalsize\sffamily\bfseries\boldmath}}
\def\subsubsection{\@startsection{subsubsection}{3}{\z@}%
    {-21dd plus-4pt minus-4pt}{10.5dd plus 4pt
     minus4pt}{\normalsize\sffamily}}
\def\paragraph{\@startsection{subsubsection}{4}{\z@}%
    {-21dd plus-4pt minus-4pt}{-1pt}{\normalsize\sffamily\bfseries}}
\def\authorfont{\rmfamily}
\def\leftlegendglue{\hfil}
\def\vec#1{\ensuremath{\mathbf{#1}}}
\journalname{EPJ}}
%%
\endinput

